Recovering Explanations from Transformed Rule-Based Ontologies

Datalog rules are often used to define ontologies over Knowledge Graphs. Rule reasoners routinely optimise such ontologies by rewriting their rules into a form that can be evaluated more efficiently. These transformations preserve the entailed facts, but not the structure of the underlying derivations. A proof tree under the rewritten rules explains why a fact holds, but does not readily yield an explanation in terms of the original rules. We study the problem of constructing, from a proof of entailment under the rewritten rules, a proof under the original ones: we establish its computational complexity and identify two practically relevant languages for specifying proof transformations.

==> macros.tex <==
\usepackage{todonotes}
\newcommand{\ale}[1]{\todo[author=AI,color=green!30,inline]{#1}}
\newcommand{\mak}[1]{\todo[author=MK,color=orange!30,inline]{#1}}
\newcommand{\mam}[1]{\todo[author=MM,color=teal!30,inline]{#1}}
\usepackage{thmtools, thm-restate}

\RequirePackage{mathtools}
\mathtoolsset{centercolon} %
\RequirePackage{xspace}

\newcommand{\ghost}[1]{\raisebox{0pt}[0pt][0pt]{\makebox[0pt][l]{#1}}}

\let\uglyphi\phi
\let\uglyepsilon\epsilon
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}

\newcommand{\ie}{i.e.,}
\newcommand{\eg}{e.g.,}
\newcommand{\cf}{cf.\,}

\hyphenation{Data-log}
\hyphenation{RDFox} %
\hyphenation{Exp-Time} %
\hyphenation{NExp-Time} %

\newcommand{\myparagraph}[1]{\vspace{1ex plus 0.5ex minus 0.5ex}\noindent\textbf{#1}~~}
\newcommand{\alglineref}[1]{L\ref{#1}} %


\newcommand{\opfont}[1]{\text{{\sf #1}}} %
\newcommand{\tuple}[1]{\langle{#1}\rangle}
\renewcommand{\vec}[1]{\bar{#1}}
\newcommand{\defeq}{\coloneqq}
\newcommand{\arity}{\opfont{ar}} %
\newcommand{\domain}[1]{\opfont{dom}(#1)} %
\newcommand{\sizeof}[1]{|#1|}
\newcommand{\factsof}[1]{\opfont{facts}(#1)}
\newcommand{\set}[1]{\{#1\}}

\newcommand{\natnum}{\ensuremath{\mathbb{N}}} %


\newcommand{\lang}[1]{\ensuremath{\mathbf{#1}}} %
\newcommand{\Clang}{\lang{C}} %
\newcommand{\Vlang}{\lang{V}} %
\newcommand{\Tlang}{\lang{T}} %
\newcommand{\Plang}{\lang{P}} %
\newcommand{\Flang}{\mathfrak{F}} %
\newcommand{\Alang}{\mathfrak{A}} %

\newcommand{\Pinput}{\Plang_{\opfont{in}}} %
\newcommand{\Poutput}{\Plang_{\opfont{out}}} %
\newcommand{\chaseoutput}{\opfont{out}} %

\newcommand{\predname}[1]{\text{{\sf #1}}} %
\newcommand{\prednamesub}[2]{\text{{\sf #1}}_\text{{\sf #2}}} %

\newcommand{\atomSet}[1]{\mathbf{#1}} %
\newcommand{\atomSetA}{\atomSet{A}}
\newcommand{\atomSetB}{\atomSet{B}}
\newcommand{\atomSetC}{\atomSet{C}}
\newcommand{\atomSetD}{\atomSet{D}}



\newcommand{\Dnter}{\mathcal{D}} %
\newcommand{\Inter}{\mathcal{I}} %
\newcommand{\Jnter}{\mathcal{J}} %


\newcommand{\aprogram}{\Pi} %
\newcommand{\arule}{\rho} %
\newcommand{\rbody}{\opfont{body}} %
\newcommand{\rbodyi}[2]{\opfont{body}_{#1}(#2)} %
\newcommand{\rbodypos}[1]{\opfont{body}^+(#1)} %
\newcommand{\rbodyneg}[1]{\opfont{body}^-(#1)} %
\newcommand{\rhead}[1]{\opfont{head}(#1)} %
\newcommand{\vars}{\opfont{vars}} %
\newcommand{\terms}{\opfont{terms}} %
\newcommand{\pout}{\opfont{out}} %

\newcommand{\orig}{\opfont{orig}} %
\newcommand{\locOrig}{\opfont{loc}} %

\newcommand{\cmps}{\opfont{cmp}} %
\newcommand{\nocmp}{\opfont{nocmp}} %
\newcommand{\fromEndPoint}[2]{#1|_{#2}} %
\newcommand{\fromNoEndPoint}[1]{#1|_{\opfont{local}}} %

\newcommand{\fnFlt}{\opfont{flt}} %
\newcommand{\fnInfFlt}{\opfont{hflt}} %



\newcommand{\complclass}[1]{\text{{\sc #1}}\xspace} %

\newcommand{\NCone}{\complclass{NC$^1$}}
\newcommand{\LogSpace}{\complclass{L}}
\newcommand{\LogCFL}{\complclass{LogCFL}}
\newcommand{\NLogSpace}{\complclass{NL}}
\newcommand{\PTime}{\complclass{PTime}}
\newcommand{\NP}{\complclass{NP}}
\newcommand{\coNP}{\complclass{coNP}}
\newcommand{\DP}{\complclass{DP}}
\newcommand{\SigmaTwoP}{\ensuremath{\Sigma_{\complclass{2}}^{\complclass{P}}}}
\newcommand{\PSpace}{\complclass{PSpace}}
\newcommand{\ExpTime}{\complclass{ExpTime}}
\newcommand{\TwoExpTime}{\complclass{2ExpTime}}
\newcommand{\kExpTime}[1]{\complclass{\ensuremath{#1}-ExpTime}}
\newcommand{\kExpSpace}[1]{\complclass{\ensuremath{#1}-ExpSpace}}

\newcommand{\etal}{\textit{et al}.}

\newcommand{\newterm}[1]{\emph{#1}} %

\newcommand{\troot}{\opfont{root}}
\newcommand{\ch}{\opfont{ch}} %
\newcommand{\tfact}{\opfont{fact}} %
\newcommand{\tatom}{\opfont{atom}} %
\newcommand{\trule}{\opfont{rule}} %
\newcommand{\mleaf}{\bot} %
\newcommand{\leafdb}[1]{\Dnter_{#1}} %
\newcommand{\unfold}{\opfont{unfold}} %
\newcommand{\tisomorph}{\cong} %


\newcommand{\enctree}{\mathsf{Tree}}
\newcommand{\encdag}{\mathsf{DAG}}
\newcommand{\enc}{\mathsf{enc}}

\newcommand{\TransTree}{\textnormal{\textsc{Trans}}_{\enctree}}
\newcommand{\TransDAG}{\textnormal{\textsc{Trans}}_{\encdag}}
\newcommand{\TransEnc}{\textnormal{\textsc{Trans}}_{\enc}}


\newcommand{\contained}{\sqsubseteq}
\newcommand{\ucontained}{\sqsubseteq_u}


\newcommand{\msochild}{\opfont{child}}
\newcommand{\msorule}{\opfont{rule}}
\newcommand{\msoarg}{\opfont{arg}}
\newcommand{\msotree}{\mathcal{I}}
\newcommand{\dbactive}{\mathcal{A}}


